Position and Velocity estimation of Re-entry Vehicles using Fast Unscented Kalman Filters

Application of two new UKF based estimation techniques with reduced processing time in re-entry vehicle position and velocity estimation problem using ground-based range and elevation measurements is presented. The first method is called the Single Propagation Unscented Kalman Filter (SPUKF) where, the a postiriori state is propagated only once and then the sampled sigma points at the next time state are approximated by the first-order Taylor Series terms. In the second method called the Extrapolated Single Propagation Unscented Kalman Filter (ESPUKF), the sigma points are approximated to the second-order Taylor Series terms using the Richardson Extrapolation. The EKF, SPUKF, ESPUKF and the UKF are utilized in a re-entry vehicle navigation scenario using range and elevation measurements. The estimation accuracies and the processing times for different algorithms are compared for the scenario. The result demonstrates that the UKF provides better accuracy than the EKF but requires more processing time. The SPUKF accuracy is better than the EKF and the processing time is significantly less than the UKF. However, the accuracy of the SPUKF is less than the UKF. The ESPUKF provides estimation accuracy comparable to the UKF and the processing time is also significantly reduced.

==> sim_assumption.tex <==
\section*{Simulation Procedure and Assumptions}
The SPIRENT GSS8000 GNSS simulator is capable of simulating GPS, GLONASS and Galileo signals. This simulator takes vehicle motion as input, generates GNSS satellites' positions from the ephemeris and simulates the signals to be received by the user GNSS-receiver from the Visible satellites. The simulator can generate tropospheric and ionospheric errors in measurements and also can incorporate receiver clock bias, if actual receiver is not available in the simulation. Figure \ref{fig:spirent} shows the basic operation of the SPIRENT simulator.
\begin{figure}[h]%
\includegraphics[width=\columnwidth]{spirent.jpg}%
\caption{SPIRENT simulator operation}%
\label{fig:spirent}%
\end{figure}
For the LEO satellite position estimation simulation without any GNSS receiver in the process, a reference orbit of the user satellite was defined in the SPIRENT GNSS simulator. Based on the reference orbit, the simulator generates GNSS signals and measurements. These measurements were recorded and used in MATLAB environment to estimate the position of the user satellite.

\subsection*{Use of Reference Orbit in SPIRENT}
\label{sec:reforb}
The SPIRENT GNSS simulator has a provision for defining the Keplerian orbit parameters to describe the orbit under consideration. These parameters are used in a pre-defined orbit model to obtain the reference position of the satellite. Another way of providing the reference orbit to the simulation scenario is directly defining the position of the satellite with respect to time. If the precise position of the satellite is known, then the second approach is more accurate than generating the reference orbit in simulation. GFZ Potsdam provides the POD solution for the TanDEM-X satellite in the Earth Centred Earth Fixed (ECEF) frame. The position data are collected and converted into a series of user motion commands which are recognised by the SPIRENT simulator.
\begin{figure}[h]%
\centering
\includegraphics[width=\textwidth]{data_conv.jpg}%
\caption{Using POD data in SPIRENT}%
\label{fig:data_C}%
\end{figure}
The POD solution provides the position of the satellite in every 120s. The SPIRENT simulator interpolates the position of the satellite during this time interval. In figure \ref{fig:data_C} the sequential process of providing reference orbit to SPIRENT is shown. This method was utilized to provide the best possible reference orbit to the simulation scenario. This reference orbit was considered as the truth and used to calculate the estimation error in the simulations. The starting epoch was selected arbitrarily at 17th December 2013.


\subsection*{GNSS measurement simulation}
\label{sub:meas}
For the GNSS signal and measurement simulations, all the 32 satellites of the GPS are considered and the full constellation of the Galileo is assumed. The SPIRENT GNSS simulator provides both pseudo-range and carrier-range data directly, when a GNSS receiver is not connected to the simulator. The receiver clock bias is simulated in the scenario. The carrier-range does not contain the integer ambiguity but, the ionospheric delay is considered and simulated in the scenario, using the default SPIRENT ionospheric delay model. The measurements are generated at 1Hz rate.

\subsection*{Model for state propagation}
In Extended Kalman Filter based Estimation technique the estimable states are propagated to calculate a priori states. In the present simulation experiment a simple orbit model is used for propagation. Following the conventional approach, the states associated with the satellite motion are selected as:
\begin{equation}
{\bf{X_{sat}}} = \begin{bmatrix}
								{\bf{r}}\\
								{\bf{v}}
								\end{bmatrix} = \begin{bmatrix}x &y &z &v_x &v_y &v_z\end{bmatrix}^T
\label{eq:eq1}
\end{equation}
where
${\bf{r}}=[x\quad y\quad z]^T$is the position vector of the satellite in the Earth Centred Inertial (ECI) frame and
${\bf{v}}=[v_x \quad v_y \quad v_z]^T$is the velocity vector of the satellite in the ECI frame.
The dynamical equation of these states includes acceleration of the satellite. As the scenario is a LEO mission, the effect of the Sun and the Moon on the acceleration are neglected. Considering $J_2$, $J_3$ and $J_4$ zonal harmonics, the acceleration of the satellite due to the Earth's gravity field in ECI frame is expressed as \cite{valladofundamentals} :
\begin{equation}
 {\bf\ddot{r}} = \begin{bmatrix}
								-\frac{\mu_ex}{r^3}(1 + J_2C_{1x}+J_3C_{2x}+J_4C_{3x})\\
								-\frac{\mu_ey}{r^3}(1 + J_2C_{1y}+J_3C_{2y}+J_4C_{3y})\\
								-\frac{\mu_ez}{r^3}(1 + J_2C_{1z}+J_3C_{2z}+\frac{mu_e}{r^2}J_3C_{3z}+J_4C_{4z})
								\end{bmatrix}
\label{eq:eq2}
\end{equation}

where
\begin{align*}
 C_{1x} =& \left(\frac{R_e}{r}\right)^2 \frac{3}{2} \left(1 - 5\frac{z^2}{r^2}\right)\\
 C_{2x} =& \left(\frac{R_e}{r}\right)^3 \frac{5}{2} \left(3 - 7\frac{z^2}{r^2}\right) \frac{z}{r}\\
 C_{3x} =& -\left(\frac{R_e}{r}\right)^4 \frac{5}{8} \left(3 - 42\frac{z^2}{r^2}+63\frac{z^4}{r^4}\right)\\
\end{align*}
\begin{align*}
 C_{1y} =& \left(\frac{R_e}{r}\right)^2 \frac{3}{2} \left(1 - 5\frac{z^2}{r^2}\right)\\
 C_{2y} =& \left(\frac{R_e}{r}\right)^3 \frac{5}{2} \left(3 - 7\frac{z^2}{r^2}\right) \frac{z}{r}\\
 C_{3y} =& -\left(\frac{R_e}{r}\right)^4 \frac{5}{8} \left(3 - 42\frac{z^2}{r^2}+63\frac{z^4}{r^4}\right)\\
 C_{1z} =& \left(\frac{R_e}{r}\right)^2 \frac{3}{2} \left(3 - 5\frac{z^2}{r^2}\right)\\
 C_{2z} =& \left(\frac{R_e}{r}\right)^3 \frac{5}{2} \left(6 - 7\frac{z^2}{r^2}\right) \frac{z}{r}\\
 C_{3z} =& \left(\frac{R_e}{r}\right)^2 \frac{3}{2}\\
 C_{4z} =& -\left(\frac{R_e}{r}\right)^4 \frac{5}{8} \left(15 - 70\frac{z^2}{r^2}+63\frac{z^4}{r^4}\right)\\
\end{align*}
and $r = \sqrt{x^2+y^2+z^2}$, $R_e$ and $\mu_e$ are the mean radius of the Earth and the gravitational parameter of the Earth respectively. The differential equation for the states can be represented as:
\begin{equation}
 {\bf\dot{X}_{sat}} = \begin{bmatrix}
												{\bf\dot{r}}\\
												{\bf\dot{v}}
												\end{bmatrix} + {\bf W_{sat}(t)} = \begin{bmatrix}
																														{\bf v}\\
																														{\bf\ddot{r}}
																														\end{bmatrix} + {\bf W_{sat}(t)}
\label{eq:eq3}
\end{equation}
Here the $\bf W_{sat}$ vector is the process noise vector which represents the unmodeled dynamics of the motion.
 Apart from the states associated with the satellite motion, the GNSS receiver clock bias and the bias rate are also considered as estimable states. The Namuru V3.3 receiver uses a single clock for both the GPS and Galileo constellations. For this reason, two states associated with the receiver clock bias are included. A receiver clock bias model can be represented as a first order Markov process. The receiver clock bias dynamics can be represented as \cite{qiao2009multiple} :
\begin{equation}
{\bf\dot{X}_{clk}} = \begin{bmatrix}
											0&1\\
											0& -\frac{1}{\nu}
											\end{bmatrix}{\bf X_{clk}} + \begin{bmatrix}
																									 w_u\\
																									 w_{ru}
																									\end{bmatrix}																									
\label{eq:eq4}
\end{equation}
where,
${\bf X_{clk}} = [\delta t_u\quad \delta t_{ru}]^T$, $\nu$ is the clock model correlation time, ${\bf W_{clk}} = [w_u\quad w_{ru}]^T$ is random noise. $\delta t_u$ is the receiver clock bias and $\delta t_{ru}$ is the receiver clock bias rate. The complete state vector and the process noise for the estimation are:
\begin{align*}
{\bf X} = \begin{bmatrix}
						{\bf X_{sat}}\\
						{\bf X_{clk}}
						\end{bmatrix} &&
{\bf W} = \begin{bmatrix}
						{\bf W_{sat}}\\
						{\bf W_{clk}}
						\end{bmatrix} &&
\end{align*}   
\subsection*{Measurement model}
Pseudo-range and carrier range measurements of the GNSS is modelled as \cite{kaplan2005understanding,Misra2006} :
\begin{equation}
\rho_{i}(t) = r_i(t) + c[\delta t_u(t) - \delta t_i(t - \tau)] + {\bf I}(t) + \epsilon_{\rho}(t)
\label{eq:eq5}
\end{equation}

\begin{equation}
\Phi_{i}(t) = r_i(t) + c[\delta t_u(t) - \delta t_i(t - \tau)] + {\bf I}(t) + \lambda N + \epsilon_{\Phi}(t)
\label{eq:eq6}
\end{equation}
where\\
\\ \begin{tabular}{cl}
 $i$ & is GNSS satellite index\\
 $\rho_i$ & is pseudo-range from the LEO satellite\\
          & to the navigation satellite $i$\\
 $\Phi_i$ & is carrier-range from the LEO satellite\\
          & to the navigation satellite $i$\\
 $r_i$ & is geometric distance from LEO satellite\\
       & to the navigation satellite $i$\\
 $\delta t$& is receiver clock bias\\
 $\delta t_i$& is clock bias of the navigation satellite\\
 $\tau$ & is signal transmission time\\
 $c$ & is velocity of light\\
 ${\bf I}(t)$& is ionospheric error\\
 $\lambda$ & is the wavelength of the carrier signal\\
 $N$ & is intiger ambiguity\\
 $\epsilon_{\rho}(t)$& is random noise in pseudo-range measurement\\
 $\epsilon_{\Phi}(t)$& is random noise in carrier-range measurement   
\end{tabular}\\

When the integer ambiguity is resolved using GRAPHIC technique \cite{jones1993environmental} , the ionospheric error can be eliminated. This method is utilized in the simulation experiments without any receiver, because the simulated carrier phase measurements in these cases, do not contain the integer ambiguity.

\subsection*{Estimation}
A conventional Extended Kalman Filter (EKF) algorithm \cite{montenbruck2000satellite} is used to estimate the states. The filter tuning parameters are the process noise covariance matrix $\bf Q$, the measurement noise covariance matrix $\bf R$ and the initial value of the state covariance matrix $\bf P$. For the initialization of the Extended Kalman Filter an initial guess of the state vector is required. The least squares method is utilized to make an initial guess of the state vector. The $\bf P$ matrix is initialized using the uncertainties calculated from least square estimation. $\bf Q$ and $\bf R$ are selected as $E[{\bf WW^T}]$ and $E[{\bf VV^T}]$. $\bf V$ is the measurement noise vector which contains all the measurement noises associated with the measurements at a particular time. Both the process noise and the measurement noise are considered as auto-correlated and not cross-correlated. This assumption results in diagonal $\bf Q$ and $\bf R$ matrices. For utilizing both the GPS and Galileo measurements a single Extended Kalman Filter is used. All the measurements from the GPS and Galileo at the same time are considered in a single measurement vector and subsequently processed through the EKF. In figure \ref{fig:EKF_iono} the estimation process is shown in block diagram.
\begin{figure}%
\includegraphics[width=\textwidth]{EKF_iono.jpg}%
\caption{Block diagram of the estimation process}%
\label{fig:EKF_iono}%
\end{figure}



==> sim_res.tex <==
\section*{Simulation result and discussion}
\label{sec:GPSGAL_EKF}
Using the described method, a Lower Earth Orbit satellite mission is simulated. POD data of TanDEM-X satellite was obtained from GFZ Potsdam and used as the reference orbit in simulation. Both GPS and Galileo constellations were simulated and the measurements are used in an Extended Kalman Filter based Algorithm to determine the satellite position. Figure \ref{fig:GPSGAL} shows the position estimation error in each axis of the ECI frame. 
\begin{figure}[!h]%
\includegraphics[width=\columnwidth]{GPS_GAL_EKF.jpg}%
\caption{Position estimation error using GPS and Galileo measurements}%
\label{fig:GPSGAL}%
\end{figure}
The root mean square error is 3.19 cm and the measurement rate is 1 Hz.
It is observed that, the simulations using only SPIRENT measurements result in satellite position estimation error within the centimetre level. This simulations use the precise position of the TanDEM-X as a reference orbit to generate the GPS as well as the Galileo signals. The receiver clock bias and the ionospheric delay were simulated and random noises were incorporated in the measurements artificially. In the EKF a simplified orbit and clock model was used. The receiver clock bias was constant and both the pseudo-range and the carrier-range measurements were used for the estimation. The constant clock bias resulted in very accurate receiver clock bias estimation using a simplified receiver clock model. Using both code and carrier phase measurements the ionospheric delay was eliminated. Also the positions of the GNSS satellites were known accurately. These assumptions resulted in centimetre level accuracy in the LEO satellite position estimation using EKF.
